Lexidate: Model Evaluation and Selection with Lexicase

Automated machine learning streamlines the task of finding effective machine learning pipelines by automating model training, evaluation, and selection. Traditional evaluation strategies, like cross-validation (CV), generate one value that averages the accuracy of a pipeline's predictions. This single value, however, may not fully describe the generalizability of the pipeline. Here, we present Lexicase-based Validation (lexidate), a method that uses multiple, independent prediction values for selection. Lexidate splits training data into a learning set and a selection set. Pipelines are trained on the learning set and make predictions on the selection set. The predictions are graded for correctness and used by lexicase selection to identify parent pipelines. Compared to 10-fold CV, lexicase reduces the training time. We test the effectiveness of three lexidate configurations within the Tree-based Pipeline Optimization Tool 2 (TPOT2) package on six OpenML classification tasks. In one configuration, we detected no difference in the accuracy of the final model returned from TPOT2 on most tasks compared to 10-fold CV. All configurations studied here returned similar or less complex final pipelines compared to 10-fold CV.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> Text/lexicase.tex <==
\section{Lexicase Selection}

A parent selection algorithm selects promising individuals (parents) from the current population, based on some quality measurement. 
These parents undergo genetic variation to construct the next generation of solutions.
We used lexicase selection \cite{helmuth2015lexicase} in this work, a popular parent selection method. % called lexicase selection \cite{helmuth2015lexicase} in this work.

% \begin{algorithm}
% \caption{Lexicase Selection}
% \label{alg:lex}
% \begin{algorithmic}[1]
% \Procedure{Lexicase}{pop, objectives}
%     % \State $parents = []$
%     % \While{$size(parents) < pop\_size$}
%         \State $curr\_pool = pop$
%         \State $shuffled\_objectives$ = Shuffle(objectives)
%         % \State $curr\_objectives$ = objectives sorted in a random order
%         \For{$obj$ in $shuffled\_objectives$}
%             \State $best\_val$ = best value on $obj$ in $curr\_pool$ 
%             \State $curr\_pool$ = inds. from $curr\_pool$ with $obj$ value as $best\_val$
%         \EndFor

%         \State \textbf{Return} $random(curr\_pool)$
%        %  \If{$size(curr\_pool \not=1)$}
%        %      \State $parents$ = $parents$ + one individual from $curr\_pool$ chosen randomly
%        %  \Else
%        %      \State $parents$ = $parents$ + $curr\_pool$
%        % \EndIf
%     % \EndWhile
% \EndProcedure

% \end{algorithmic}
% \end{algorithm}


Generally, lexicase selection takes a list of individuals and their scores on a set of objectives (also called test cases) as input. 
To select an individual parent, the whole population is placed into the selection pool. 
Next, the set of test cases is randomly shuffled, and each test case is used to remove individuals from the selection pool;
individuals which do not have the best score from the current selection pool on the test case are removed. %who are not best on that test case.
This process is repeated until we run out of test cases.
If multiple individuals remain, one is randomly returned as a parent.
Algorithm \ref{alg:lex} presents the pseudocode for lexicase selection adapted from ~\cite{ribeiro2024tpot2}. 

% As discussed earlier, a parent selection method in a given evolutionary run is used to select individuals from the current generation, based on some criteria, that are used to produce the next generation of individuals through genetic variation. 
% In the experiments described in this paper, we use a selection method called Lexicase selection~\cite{helmuth2015lexicase}. 
% In its most general form, it takes in as input a list of current individuals and their scores on a set of objectives (also called test cases). The following procedure is followed for selecting each parent. 
% Initially, the whole population is put into the selection pool. We first randomly shuffle the objectives. 
% Then, the individuals which are best on the first test case are kept in the pool and the rest are removed. 
% Then the individuals which are best on the second test case are kept and the rest are removed. 
% The process is repeated until we are left with one individual, or if we are left with multiple individuals after exhausting the objectives, we select one individual at random to be returned as a parent. 
% Algorithm \ref{alg:lex} presents the pseudocode for lexicase selection, adapted from ~\cite{ribeiro2024tpot2}. 





% \subsection{Lexicase for program synthesis}

% Inductive program synthesis, or Programming-by-examples, is a sub-field of program synthesis that aims to automatically create computer programs that match a given set of input/output examples. 
% When lexicase selection is used in genetic programming for these kinds of problems, examples of expected input and output form the objectives used during selection.
% In other words, lexicase selection takes a list of performances on these examples as input (\textit{e.g.}, the difference between actual output values and the predicted output values for each example input/output case).
% These performances can be binary or real-valued. 
% The errors can be binary (whether the actual and predicted outputs match), or real-valued. 
% Objectives not related to performance can also be used, such as program size, presence of looping instructions, and uniqueness in the population~\cite{saini2020using}. 

% Inductive program synthesis, also known as Programming-by-examples, is a subfield of program synthesis that aims to automatically create programs that match a given set of input/output examples. 
% When lexicase selection is used for this purpose in genetic programming, these `examples' form the objectives used during selection. 
% In other words, the input to lexicase selection is the list of errors on these examples, i.e., the difference between actual output values and the predicted output values for each of the input/output pairs. 
% The errors can be binary (whether the actual and predicted outputs match), or real-valued. Other objectives related to the individuals such as program size, presence of looping instructions, etc., can also be used with lexicase selection [CITE]. 

\subsection{Lexicase for TPOT} 

In the prior work, lexicase selection has been modified for an AutoML setting within TPOT.
The fitness of a pipeline is the aggregated differences between the actual output and its predicted output. 
% For a given pipeline, the fitness value was calculated as the aggregated differences between the actual output and the predicted output of a pipeline. 
The fitness value is aggregated on two levels. 
When using the $k$-fold cross-validation, the $k$ scores calculated from each fold are averaged, where each of the $k$ scores is an aggregate value of some evaluation metric (\textit{e.g.}, accuracy, f1 score, \textit{etc.}). 
Pipeline properties are also used as objectives, such as number of nodes and complexity in terms of learnable parameters~\cite{matsumoto2023faster,ribeiro2024tpot2}. 
% Other properties of individual pipelines such as size, etc. are also used as other objectives. 
Typically, two fitness values are assigned to each pipeline with TPOT and TPOT2: a cross-validation score on the training set and pipeline complexity. 
% For TPOT2, therefore, in most cases, we have two fitness values for every pipeline: average cross-validation score on the training set, and complexity (e.g., size) of the pipeline. 
Although lexicase selection has a faster rate of convergence than NSGA2 with these two objectives (as described above)~\cite{matsumoto2023faster}, its benefits with de-aggregated objectives have not been studied in the AutoML space. % in the literature. 
% Although lexicase selection performs better than NSGA2 in terms of the rate of convergence with two objectives (as described above)~\cite{matsumoto2023faster}, its benefits with de-aggregated objectives have not been studied in the AutoML space in the literature. 
Lexicase selection, as used in TPOT and TPOT2, deviates from its initially intended design: consider all particular cases and combinations of cases, and explore their implications independently while not averaging them~\cite{spector2023particularity}. 
% Although even with two objectives, lexicase selection seems to perform better than NSGA2 in terms of the rate of convergence [CITE], its benefits with de-aggregated objectives have not been studied in the AutoML space in the literature. 
% Lexicase selection as used in TPOT and TPOT2 is quite removed from how it was originally designed to be used:  consider all particular cases and combinations of cases, and explore their implications as independently as possible while avoiding averaging over them~\cite{spector2023particularity}. 
Lexidate offers a method for incorporating lexicase selection into evolutionary AutoML that aligns more closely with its original design.

==> Text/tpot2.tex <==
\section{TPOT2}

In our experiments, we used the Tree-based Pipeline Optimization Tool (TPOT)~\cite{olson2016tpot}, an AutoML tool that implements a genetic programming system to evolve machine learning pipelines.
These pipelines consist of a sequence of machine learning methods (\textit{e.g.}, feature selection, feature transformation, classification, regression, \textit{etc.}) that are executed in some order.
Specifically, we use TPOT2~\cite{ribeiro2024tpot2} (\textit{i.e.}, the next iteration of TPOT) where pipelines are represented as directed-acyclic graphs. 
Pipelines in TPOT2 are composed of three node types: leaf, inner, and root nodes. 
Each node encodes a machine learning model and its parameters.
Users can specify the kinds of models for each node type, the number of nodes in a pipeline, and restrictions on the topology of a pipeline's graph.
The leaf nodes receive data as input, and their output is passed to the inner nodes or the root node.
The inner nodes operate on the output of the leaf nodes or other inner nodes, and pass their output to the following inner nodes or the root node. 
Pipelines are restricted to a single root node which is a classification or regression model.
Figure \ref{fig:tpot2_example} demonstrates an example pipeline in TPOT2.

\begin{figure}[h]
\includegraphics[width=\linewidth]{Figures/tpot2_example.png}
\caption{A typical individual pipeline represented in TPOT2.}
\label{fig:tpot2_example} 
\end{figure}

% In our experiments, we use an automated machine learning (AutoML) tool called Tree-based Pipeline Optimization Tool (TPOT)~\cite{olson2016tpot}. 
% It is a genetic programming system to evolve machine learning pipelines. 
% An ML pipeline (or, pipeline for short) is a sequence of ML methods related to feature selection, feature transformation, classification, regression, etc., that are executed in some order on a given dataset. 
% In particular, we use the next iteration of TPOT called TPOT2~\cite{ribeiro2024tpot2} in which pipelines are represented as directed-acyclic graphs (DAGs). 
% A typical TPOT2 individual contains three types of nodes: leaf nodes, inner nodes, and a root node. 
% Each node encodes for an ML model as well as its parameters. Whereas the user can specify the possible ML models for each type of node, the exact number of nodes and the structure of the graph for an individual are determined by the evolution. 
% The leaf nodes have access to the dataset and their output is passed on to the next inner node or directly to the root node. 
% The inner nodes operate on the output of the leaf nodes and pass their output to the root node. 
% The graph individual has only one root node which is typically the final classifier or regression model. Figure \ref{fig:tpot2_example} shows an example of how various nodes in a TPOT2 individual might be structured.

\subsection{Evolutionary algorithm}

TPOT2 evolves pipelines in the following manner.
The first generation is populated with $pop\_size$ randomly generated pipelines, where $pop\_size$ is the size of a population specified by a user.
After the first population is constructed, pipelines are evaluated based on the given problem, data set, and user-specified evaluation metrics (objective functions).
During model evaluation, invalid pipelines and pipelines that exceed a user-specified time limit may arise.
These solutions are removed from the population.
Once all pipelines are evaluated, survival selection is used to identify $pop\_size$ survivors, where all pipelines are survivors in the first generation.
A parent selection method is then used to identify $pop\_size$ promising parents from the set of survivors.
These parent pipelines are varied through a combination of mutation and crossover to produce offspring, where offspring are evaluated like their parents.
The combination of offspring and survivors (size of $2*pop\_size$) is then passed to survivor selection to identify $pop\_size$ survivors, and the cycle continues.



The cycle repeats for a user-specified number of generations, or until enough generations pass and no progress is made.
At the end of a run, the \textit{best} pipeline is identified from all the evaluated individuals.
First, all pipelines that performed best on the first objective function are gathered. 
If more than one objective function was used, the next objective is used to filter out those pipelines from the current subset that did not perform best.
We repeat this process until all objectives are used and return a random pipeline if multiple pipelines remain.

% The process is repeated for a certain number of generations as specified by the user.
% At the end of the run, we determine the \textit{best} individual from all the evaluated individuals using the following process. 
% We first find the list of individuals which are best on the first objective function. 
% Out of them, we keep only the individuals which are best on the second objective function, and delete the rest. 
% We repeat this process until we find one individual, or if there are many left, we choose one randomly from the remaining ones.
